Implicit representation priors meet Riemannian geometry for Bayesian robotic grasping

Robotic grasping in highly noisy environments presents complex challenges, especially with limited prior knowledge about the scene. In particular, identifying good grasping poses with Bayesian inference becomes difficult due to two reasons: i) generating data from uninformative priors proves to be inefficient, and ii) the posterior often entails a complex distribution defined on a Riemannian manifold. In this study, we explore the use of implicit representations to construct scene-dependent priors, thereby enabling the application of efficient simulation-based Bayesian inference algorithms for determining successful grasp poses in unstructured environments. Results from both simulation and physical benchmarks showcase the high success rate and promising potential of this approach.

==> bayesian_network.tex <==
\begin{tikzpicture}[scale=1]
  % Define nodes
 % H
 \node[latent, minimum size=1cm] (h) {$\mathbf{h}$};
 
 % Z
 \node[latent, right=2cm of h, minimum size=1cm] (z) {$\mathbf{z}$};
 
 % V
 \node[obs, below=1cm of z, minimum size=1cm]  (P) {$\mathbf{P}$};
 
  % S
  \node[obs, below=1cm of h, minimum size=1cm] (S) {$S$};
  
  % Connect the nodes
  \edge{h, z}{S};
  \edge{z}{P};
  \edge{P}{h};
  \edge{P}{S};
 
 % Define nodes

 % H
  %\node[det, fill=gray!25, minimum size=1.6cm] (hv) {$\mathbf{h}$};
  % X, R and g
  %\node[obs, above=1cm of hv, minimum size=1cm] (R) {$\mathbf{q}_{\text{P}}$};
  %\node[obs, above=1cm of hv, xshift=-1.2cm, minimum size=1cm] (x) {$\mathbf{x}_{\text{P}}$};
  %\node[obs, above=1cm of hv, xshift=1.2cm, minimum size=1cm] (g) {$g$};
  % Edge
  %\edge{x, R, g}{hv};
  
  % T_LO
  %\node[det, right=2.5cm of hv, minimum size=1.6cm] (pO) {$\mathbf{T_{\mathrm{DO}}}$};
  %\node[latent, above=1cm of pO, xshift=-1.2cm, minimum size=1cm] (xO) {$x_{\mathcal{O}}$};
  %\node[latent, above=1cm of pO, minimum size=1cm] (yO) {$y_{\mathcal{O}}$};
  %\node[latent, above=1cm of pO, xshift=1.2cm, minimum size=1cm] (rO) {$\varphi_{z, \mathcal{O}}$};
  %\edge{xO, yO, rO}{pO};
 
  
  % Object
  %\node[det, right=2.5cm of pO, minimum size=1.6cm] (Ov) {$\mathrm{Object}$};
  %\node[latent, above=1cm of Ov, xshift=-0.6cm, minimum size=1cm] (M) {$\mathcal{O}$};
  %\node[latent, above=1cm of Ov, xshift=0.6cm, minimum size=1cm] (scale) {$\beta$};
  %\edge{M, scale}{Ov};
  %\edge{Ov}{pO};
  
  
  

  % S
  %\node[obs, below=1cm of hv, minimum size=1cm] (S) {$S$};
  % i
  %\node[obs, below=1cm of pO, minimum size=1cm]  (i) {$i$};
  % T_BC
  %\node[det, fill=gray!25, below=1cm of Ov, minimum size=1cm] (pc) {$\mathbf{T}_{\text{BC}}$};
  
  %\node[latent, left=0.5cm of S, minimum size=1cm] (fric) {$\mu$};

  % Connect the nodes
  %\edge{hv, pO, Ov}{S};
  %\edge{pO, Ov}{i};
  %\edge{pc}{i};
  %\edge{fric}{S};
  
  % Plate
  %\plate {ik} {(i)(pc)} {N};
  
\end{tikzpicture}
